Transmission Power Control for Remote State Estimation in Industrial Wireless Sensor Networks

Novel low-power wireless technologies and IoT applications open the door to the Industrial Internet of Things (IIoT). In this new paradigm, Wireless Sensor Networks (WSNs) must fulfil, despite energy and transmission power limitations, the challenging communication requirements of advanced manufacturing processes and technologies. In industrial networks, this is possible thanks to the availability of network infrastructure and the presence of a network coordinator that efficiently allocates the available radio resources. In this work, we consider a WSN that simultaneously transmits measurements of Networked Control Systems' (NCSs) dynamics to remote state estimators over a shared packet-erasure channel. We develop a minimum transmission power control (TPC) policy for the coordination of the wireless medium by formulating an infinite horizon Markov decision process (MDP) optimization problem. We compute the policy using an approximate value iteration algorithm and provide an extensive evaluation of its parameters in different interference scenarios and NCSs dynamics. The evaluation results present a comprehensive characterization of the algorithm's performance, proving that it can flexibly adapt to arbitrary use cases.

==> sections/markus-formulation.tex <==
\newpage
\section{Markus Formulation}

\samuele{to be checked...actually could be interesting to see how bad this is as an approximation of the value iteration!}

\lemma{
	The optimal cost function $J^*(P)$ can be written as $J^*(P) = \sum_\ell J_\ell^*(P)$ and each $J_\ell^*(P)$ satisfies 
	\begin{equation}
	J_\ell^*(P_\ell)= \E \left[\rho_\ell \left( P_\ell, \kappa_{k,\ell}^*\right) + \alpha J_\ell^*\left( \phi_\ell \left( P_\ell, \kappa_{k,\ell}^*\right) \right) \right] \hspace{0.2cm}\forall \ell,
	\end{equation}
	where $\vec{\kappa}_k^*$ is the solution to \eqref{eq:dyn_prog_op}.
}
\begin{IEEEproof}
	From \cite[Prop. 1.2.1]{Bertsekas_DP}, it is known that the optimal cost function converges as $J^*(P) = \lim_{N\to\infty}(T^NJ)(P)$ from any initial $J(P)$. Without loss of generality we can assume $J(P) = 0$. Using $\vec{\kappa}_k^*$ as the solution to \eqref{eq:dyn_prog_op} in each time step and defining $P_{N,\ell} = P_\ell$ $\forall \ell$, this leads to
	\begin{equation}
	(T^NJ)(P) = \E \left[ \sum_{k=0}^{N} \sum_{\ell=1}^{L} \alpha^{N-k} \rho_\ell \left( P_{k,\ell}, \vec{\kappa}_k^* \right) \right].
	\end{equation}
	Hence, we get that 
	\begin{align}
	&J^*(P) = \lim_{N\to\infty}(T^NJ)(P)\\
	&=\lim_{N\to\infty}\E \left[ \sum_{k=0}^{N} \sum_{\ell=1}^{L} \alpha^{N-k} \rho_\ell \left( P_{k,\ell}, \vec{\kappa}_k^* \right) \right]\\
	&= \lim_{N\to\infty}\E \left[\sum_{\ell=1}^{L} \left(\rho_\ell \left( P_\ell, \vec{\kappa}^* \right) +\sum_{k=0}^{N-1} \alpha^{N-k} \rho_\ell \left( P_{k,\ell}, \vec{\kappa}_k^* \right)\right) \right]\notag\\
	&= \E \left[\sum_{\ell=1}^{L} \left(\rho_\ell \left(P_\ell, \vec{\kappa}^* \right) +\alpha\lim_{N\to\infty}\sum_{k=0}^{N-1} \alpha^{N-k-1} \rho_\ell \left( P_{k,\ell}, \vec{\kappa}_k^* \right)\right) \right]\notag\\
	&=\sum_{\ell=1}^{L} \E \left[\rho_\ell \left( P_{k,\ell}, \vec{\kappa}_k^* \right) + \alpha J_\ell^*(\phi_\ell \left( P_\ell, \kappa_{k,\ell}^*\right)) \right].\label{eq:J_decomposed}
	\end{align}
	The claim holds by identifying $J_\ell^*(P_\ell)$ as the summands given in equation \eqref{eq:J_decomposed}.
\end{IEEEproof}

\markus{With this lemma, the remaining proofs should be valid for the multi-loop case!}

(Eq. 35 single-loop) - Proposition 3: The optimal stationary packet success rate policy is given by


\begin{align}
\vec{\kappa}^* &= \argmin_{\vec{\kappa} \in \Lambda} \left[ \sum_{\ell=1}^{L} \rho_\ell \left( P_\ell, \vec{\kappa}\right) + \alpha (1 - \kappa_\ell) J_\ell^*(0) + \alpha \kappa_\ell J_\ell^*(1)\right]\label{eq:opt_kappa}
\end{align}

where $J_\ell^*(\delta)= J_\ell^* \left( \tilde{F}_\ell \tilde{P}_\ell \tilde{F}_\ell^\top + R_{1,\ell} -\delta \tilde{K}_{k,\ell} \tilde{H}_\ell \tilde{P}_\ell \tilde{F}_\ell^\top\right)$.

At each $k$, the communication network will optimize \eqref{eq:opt_kappa} over $\vec{\kappa}$. Note that $\lambda_\ell \tr(\tilde{\Theta}_\ell {P}_\ell$ is independent of $\vec{\kappa}$:
\begin{align}
\rho_\ell \left( P_\ell, \vec{\kappa}\right) = \vec{\Psi}_\ell (\vec{\kappa}) + \underbrace{\lambda_\ell \tr(\tilde{\Theta}_\ell {P}_\ell)}_{\text{independent of } \vec{\kappa}}.
\end{align}

Because of this and the relationship $\vec{p}=\vec{\Psi}_\ell \left(\vec{\kappa}\right)$ $\Leftrightarrow$ $\vec{\kappa} = \vec{\text{PSR}}(\vec{p})$, the optimization problem of \eqref{eq:opt_kappa} can be equivalently formulated as:
\begin{align}
&\min_{\vec{\kappa} \in  \Lambda} \left[\sum_{\ell=1}^{L} \vec{\Psi}_\ell \left(\vec{\kappa}\right) + \alpha \kappa_\ell \left(J_\ell^*(0) - J_\ell^*(1)\right)\right]\\
\stackrel{\Delta}{=}\quad&\min_{\vec{p} \in  \mathcal{P}} \left[ \sum_{\ell=1}^{L} p_\ell - \alpha \sum_{\ell=1}^{L} \text{PSR}_\ell (\vec{p}) \left(J_\ell^*(1) - J_\ell^*(0)\right) \right]\\
\stackrel{\Delta}{=}\quad&\max_{\vec{p} \in  \mathcal{P}} \left[ \alpha \sum_{\ell=1}^{L} \text{PSR}_\ell (\vec{p}) \left(J_\ell^*(1) - J_\ell^*(0)\right) -\sum_{\ell=1}^{L} p_\ell \right]
\end{align}

\lemma{\label{lemma-4}
	The optimal stationary network transmission power policy $\vec{p}^*$, calculated using Eq.~\eqref{eq:foschini_alg}, is monotonic with respect to the optimal stationary packet success rate policy $\vec{\kappa}^*$ $\forall L$ and is the \underline{same} for all the transmitters, if
	
	\begin{itemize}
		\item[W]: the \emph{distances ($d_\ell$)} of the different transmitter-receiver pairs are the \underline{same}
		\item[W]: the \emph{avg. propagation coefficients ($\eta_\ell,\sigma^2_\ell$)} of the different transmitter-receiver pairs are the \underline{same}
		\item[C]: the \emph{control loops ($F_\ell,H_\ell,R_{1,\ell},R_{2,\ell}$)} are the \underline{same}
		\item[C]: the \emph{levels of distortion ($\beta_\ell \rightarrow \alpha_\ell, \lambda_\ell$)} of the control loops are the \underline{same}
		\item[C]: at a given time step $k$, the \emph{estimation covariances} ($P_\ell$) of the control loops are the \underline{same}, therefore \emph{stationary packet success rate policy} $\vec{\kappa}^*$ is the \underline{same} for the control loops 
		\item[W]: the \emph{stationary packet success rate policy} $\vec{\kappa}^*$ is \underline{feasible} ($\vec{\kappa} \in \Lambda$)
	\end{itemize}
	Therefore, the minimum stationary network transmission policy is obtained by solving Eq.~\eqref{eq:opt_kappa} and Eq.~\eqref{eq:foschini_alg}.
}
\begin{IEEEproof}
	If blablabla then blabla so bla!
\end{IEEEproof}

\lemma{
	Under the conditions of Lemma~\ref{lemma-4}, all the stationary packet success rate policies $\vec{\kappa}$ are feasible if the stationary packet success rate policy corresponding to the \emph{maximum} value of the estimation covariance $P_\ell$ is feasible.
}
\begin{IEEEproof}
	If blablabla then blabla so bla!
\end{IEEEproof}

%Internal use:
%
%\begin{align}
%	\mathcal{U}_i(\gamma_i) &= \alpha \kappa_\ell(\gamma_\ell) w_\ell \text{, where } w_\ell=\left(J_\ell^*(0) - J_\ell^*(1)\right)\\
%	\Rightarrow \quad& \max_{ \vec{p}, \vec{\gamma}} \quad \sum_{\ell=1}^{L} \mathcal{U}_\ell(\gamma_\ell) - \sum_{\ell=1}^{L} p_\ell\\
%	\text{s.t.}\quad & \gamma_\ell \le \text{SINR}_\ell (\vec{p})\\
%	& \vec{p} \in \mathcal{P}
%\end{align}

